Characterizing Stereotypical Bias from Privacy-preserving Pre-Training

Differential Privacy (DP) can be applied to raw text by exploiting the spatial arrangement of words in an embedding space. We investigate the implications of such text privatization on Language Models (LMs) and their tendency towards stereotypical associations. Since previous studies documented that linguistic proficiency correlates with stereotypical bias, one could assume that techniques for text privatization, which are known to degrade language modeling capabilities, would cancel out undesirable biases. By testing BERT models trained on texts containing biased statements primed with varying degrees of privacy, our study reveals that while stereotypical bias generally diminishes when privacy is tightened, text privatization does not uniformly equate to diminishing bias across all social domains. This highlights the need for careful diagnosis of bias in LMs that undergo text privatization.

==> old.tex <==

%%%%%

Differential Privacy (DP) \citep{dwork2006calibrating} transitioned from the field of statistical databases into machine learning \citep{song2013stochastic, bassily2014private, abadi2016deep, shi2022selective}. DP operates on the principle of injecting additive noise so that model outputs are indistinguishable within the bounds of a privacy budget $\varepsilon > 0$, where $\varepsilon \rightarrow \infty$ represents no bound on the information leakage. 

%\citet{abadi2016deep} integrate DP into stochastic gradient descent \citep{robbins1951stochastic}. By calculating per-example gradients \citep{goodfellow2015efficient} and adding random noise to these gradients with a scale proportional to a clipping norm, this technique effectively establishes a noise floor that strictly bounds the unique signals from any training example. However, calculating per-example gradients, while essential for privacy, can substantially slow down training speed \citep{subramani2021enabling, bu2021fast}, thereby imposing a limit to the scaling of LMs \citep{kaplan2020scaling}.

Equipped with a discrete vocabulary set $\mathcal{W}$, an embedding function $\phi : \mathcal{W} \rightarrow \mathbb{R}$, and a distance metric $d: \mathbb{R} \times \mathbb{R} \rightarrow [0,\infty)$, \citet{feyisetan2020privacy} formulated a randomized mechanism for text-to-text privatization grounded in metric differential privacy \citep{chatzikokolakis2013broadening}. Specifically, the randomized mechanism perturbs each word in a text by adding noise to the representation of the word derived from an embedding space \citep{mikolov2013efficient} and projecting the noisy representation back to a discrete vocabulary using a nearest neighbor search. Since metric differential privacy scales the notion of indistinguishability by a distance $d(\cdot)$, this technique offers several benefits: (1) It ensures that the log-likelihood ratio of observing any substitution $\hat{w}$ given two words $w$ and $w’$ is bounded by $\varepsilon d\{\phi(w), \phi(w')\}$, providing plausible deniability \citep{bindschaedler2017plausible} with respect to all $w \in \mathcal{W}$. (2) It produces similar substitutions $\hat{w}$ for any words $w$ and $w'$ that are close in the embedding space, alleviating the curse of dimensionality associated with randomized response \citep{warner1965randomized}.


•	word embedding association test (WEAT, Caliskan et al. 2017)
•	May et al. (2019) extend WEAT to sentence encoders, calling it the Sentence Encoder Association Test (SEAT).
•	Open-Ended Language Generation Dataset (BOLD) a large-scale dataset that consists of 23,679 English text generation prom
•	pts for bias benchmarking across five domains: profession, gender, race, religion, and political ideology. -> Polarity, toxicity of a continued prompt

